PLaD: Preference-based Large Language Model Distillation with Pseudo-Preference Pairs

Large Language Models (LLMs) have exhibited impressive capabilities in various tasks, yet their vast parameter sizes restrict their applicability in resource-constrained settings. Knowledge distillation (KD) offers a viable solution by transferring expertise from large teacher models to compact student models. However, traditional KD techniques face specific challenges when applied to LLMs, including restricted access to LLM outputs, significant teacher-student capacity gaps, and the inherited mis-calibration issue. In this work, we present PLaD, a novel preference-based LLM distillation framework. PLaD exploits the teacher-student capacity discrepancy to generate pseudo-preference pairs where teacher outputs are preferred over student outputs. Then, PLaD leverages a ranking loss to re-calibrate student's estimation of sequence likelihood, which steers the student's focus towards understanding the relative quality of outputs instead of simply imitating the teacher. PLaD bypasses the need for access to teacher LLM's internal states, tackles the student's expressivity limitations, and mitigates the student mis-calibration issue. Through extensive experiments on two sequence generation tasks and with various LLMs, we demonstrate the effectiveness of our proposed PLaD framework.

==> 08_checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}



==> table/add_exp.tex <==
\begin{table*}[!htb]
    \centering
    \caption{Student model's test accuracy ($\%$) on MNLI dataset with different-sized teachers. Each entry reports the average result and the standard deviation of three runs. The last column reports the results averaged on all the three settings.}
     \scalebox{1.25}{
    \begin{tabular}{c|c|c|c|c}\toprule
        Teacher Size & T5-xxl & T5-xl & T5-large & Average \\\midrule
        KL  & 90.26 \pm 0.24  &   90.38 \pm 0.06   &89.96 \pm 0.05 & 90.20 \pm 0.23  \\
        Temp.& 90.66 \pm 0.14 & 90.32 \pm 0.06  &90.38 \pm 0.03 &90.45 \pm 0.17  \\
        Smoothing & 90.63 \pm 0.43& 90.09 \pm 1.00 & 90.65 \pm 0.19 & 90.46 \pm 0.62 \\
        Focal & 90.69 \pm 0.34&89.79 \pm 0.87   & 90.30 \pm 0.05 &90.26 \pm 0.61 \\
        FilterKD & 90.68 \pm 0.18 &  89.52 \pm 0.17 & 90.24 \pm 0.19 &90.15 \pm0.53 \\
        Flooding & 90.55 \pm 0.42 &90.27 \pm 0.24   & 90.01 \pm 0.60 & 90.27 \pm 0.45  \\\midrule
        \ours & \bf91.07 \pm \bf0.07 &   \bf 90.84 \pm \bf0.11& \bf90.67 \pm \bf0.05 & \bf90.86 \pm \bf0.19\\\bottomrule
    \end{tabular}
    }
    \label{tab:add_res}
\end{table*}

==> table/main_res_beta.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c|cccccc}\toprule
       Dataset & Architecture & \cellcolor[]{gray} Temperature & Lable Smoothing & Focal & KL & PKD & PKD-eq  \\\midrule
        % \multirow{3}{*}{MNLI} & xxl& 90.07& 90.56& 90.71& 90.04& 90.92& 91.22\\
        MNLI & xxl& 90.07& 90.56& 90.71& 90.04& 90.92& 91.22\\\midrule
        % & xl&\\
        % & large&\\\midrule
        SST-2 & xxl&89.56& 89.67&89.79& 89.22& 90.59& 90.76\\\midrule
        BoolQ & xxl & 70.02& 70.40& 70.27& 69.57& 70.97& 71.87\\\bottomrule
        % & xl& 89.56& 89.67&89.79& 89.22& 90.59& 90.76\\
        % & large&\\\midrule
        % \multirow{3}{*}{BoolQ} & xxl&\\
        % & xl&\\
        % & large&\\\midrule
    \end{tabular}
    \caption{Main Results on three datasets, distilled from different-size teachers. We list the hyper-parameter search space of each method in Appendix.}
    \label{tab:main_res_beta}
\end{table}

==> table/main_res_extend.tex <==
\begin{table*}[!th]
     % \vspace{-10pt}
    \centering
     \caption{Quantitative results on natural language datasets. The student model is distilled from teacher models with different sizes. We report the student model's test accuracy ($\%$) and list the teacher model's validation accuracy ($\%$) in the colored column for reference. ``TS'' stands for temperature scaling and ``LS'' stands for Label Smoothing. We use underscore ``$\_$'' to highlight the best baseline method and use $^{*}$ ($^{**}$) to indicate the performance improvement is significant under the two-tailed paired $t$-test with 90\% (95\%) confidence level.
     }
    \scalebox{.745}{
\begin{tabular}{c|c|c|cccccc|c}\toprule
       \multirow{2}{*}{Dataset} & Teacher & Teacher & \multirow{2}{*}{KL} & \multirow{2}{*}{TS} & \multirow{2}{*}{LS} & \multirow{2}{*}{Focal} & \multirow{2}{*}{FilterKD} & \multirow{2}{*}{Flooding}  & \multirow{2}{*}{\ours}  \\
        & Size & Acc. &  &  &  &  &  &   &   \\
        \midrule        
        \multirow{3}{*}{SST-2} & XXL & \cellcolor{apricot} 96.44   & 89.18$\pm$0.3 & 89.37$\pm$0.2& \underline{89.91}$\pm$0.3  & 89.33$\pm$0.3 & 89.28$\pm$0.2 & 89.30$\pm$0.4 & \textbf{90.29}$^{*}\pm$0.1\\
                               & XL  & \cellcolor{apricot} 95.18   & 89.22$\pm$0.6 & 89.33$\pm$0.4 & \underline{90.02}$\pm$0.4  & 89.45$\pm$0.2 & 89.24$\pm$0.2&
                               89.22$\pm$0.4 & \textbf{90.10} $\pm$0.1\\
                               & Large & \cellcolor{apricot} 95.53 & 88.80$\pm$0.1 & 89.18$\pm$0.5 & 89.22$\pm$0.4  & \underline{89.26}$\pm$0.5 & 89.21$\pm$0.3&
                               88.97$\pm$0.4& \textbf{90.02}$^{**}\pm$0.2\\
        \midrule
        \multirow{3}{*}{MNLI} & XXL & \cellcolor{apricot} 94.68    & 90.26$\pm$0.2 & 90.66$\pm$ 0.1 & 90.63$\pm$0.4 & \underline{90.69}$\pm$0.3 & 90.68$\pm$0.2 & 90.55$\pm$0.4 & \textbf{91.07}$^{*}\pm$0.1 \\
                             & XL & \cellcolor{apricot} 92.42      & \underline{90.38}$\pm$0.1 & 90.32$\pm$0.1 & 90.09$\pm$1.0 & 89.79$\pm$0.9 & 89.52$\pm$0.2 & 90.27$\pm$0.2 & \textbf{90.84}$^{**}\pm$0.1\\
                             & Large  & \cellcolor{apricot} 93.56   & 89.96$\pm$0.1 & 90.38$\pm$0.1 & \underline{90.65}$\pm$0.2 & 90.30$\pm$0.1 & 90.24$\pm$0.2 & 90.01$\pm$0.6 & \textbf{90.67}$\pm$0.1\\
                             % MNLI Ave. & & & 90.20\pm0.23&90.45\pm0.17&90.46\pm0.62&90.26\pm0.61&90.15\pm0.53&90.27\pm0.45&\bf90.86\pm \bf0.19\\
        \midrule
        \multirow{3}{*}{BoolQ} & XXL  & \cellcolor{apricot} 89.14  & 69.44$\pm$0.2 & \underline{72.04}$\pm$0.3 & 68.63$\pm$0.4  & 68.18$\pm$1.5  & 69.64$\pm$0.9 & 69.26$\pm$0.5 & \textbf{73.08}$^{**}\pm$0.5\\
          & XL  & \cellcolor{apricot} 87.52  & 70.46$\pm$0.1 & \underline{72.01}$\pm$0.7 & 68.87$\pm$0.7  & 68.26$\pm$1.2  & 69.89$\pm$0.5 & 69.19$\pm$0.4 & \textbf{72.77}$^{**}\pm$0.2\\
                               & Large &  \cellcolor{apricot} 77.91 & 69.53$\pm$0.2 & \underline{70.43}$\pm$0.6 & 69.11$\pm$1.2  & 68.86$\pm$0.5 &  69.25$\pm$0.6 & 68.92$\pm$0.6 & \textbf{71.03}$^{*}\pm$0.3\\
         \midrule
         \multirow{3}{*}{RTE} & XXL  & \cellcolor{apricot} 89.14  & 69.44$\pm$0.2 & \underline{72.04}$\pm$0.3 & 68.63$\pm$0.4  & 68.18$\pm$1.5  & 69.64$\pm$0.9 & 69.26$\pm$0.5 & \textbf{73.08}$^{**}\pm$0.5\\
          & XL  & \cellcolor{apricot} 87.52  & 70.46$\pm$0.1 & \underline{72.01}$\pm$0.7 & 68.87$\pm$0.7  & 68.26$\pm$1.2  & 69.89$\pm$0.5 & 69.19$\pm$0.4 & \textbf{72.77}$^{**}\pm$0.2\\
                               & Large &  \cellcolor{apricot} 77.91 & 69.53$\pm$0.2 & \underline{70.43}$\pm$0.6 & 69.11$\pm$1.2  & 68.86$\pm$0.5 &  69.25$\pm$0.6 & 68.92$\pm$0.6 & \textbf{71.03}$^{*}\pm$0.3\\
          \midrule
         \multirow{3}{*}{MRPC} & XXL  & \cellcolor{apricot} 89.14  & 69.44$\pm$0.2 & \underline{72.04}$\pm$0.3 & 68.63$\pm$0.4  & 68.18$\pm$1.5  & 69.64$\pm$0.9 & 69.26$\pm$0.5 & \textbf{73.08}$^{**}\pm$0.5\\
          & XL  & \cellcolor{apricot} 87.52  & 70.46$\pm$0.1 & \underline{72.01}$\pm$0.7 & 68.87$\pm$0.7  & 68.26$\pm$1.2  & 69.89$\pm$0.5 & 69.19$\pm$0.4 & \textbf{72.77}$^{**}\pm$0.2\\
                               & Large &  \cellcolor{apricot} 77.91 & 69.53$\pm$0.2 & \underline{70.43}$\pm$0.6 & 69.11$\pm$1.2  & 68.86$\pm$0.5 &  69.25$\pm$0.6 & 68.92$\pm$0.6 & \textbf{71.03}$^{*}\pm$0.3\\
        \midrule
         \multirow{3}{*}{ANLI} & XXL  & \cellcolor{apricot} 89.14  & 69.44$\pm$0.2 & \underline{72.04}$\pm$0.3 & 68.63$\pm$0.4  & 68.18$\pm$1.5  & 69.64$\pm$0.9 & 69.26$\pm$0.5 & \textbf{73.08}$^{**}\pm$0.5\\
          & XL  & \cellcolor{apricot} 87.52  & 70.46$\pm$0.1 & \underline{72.01}$\pm$0.7 & 68.87$\pm$0.7  & 68.26$\pm$1.2  & 69.89$\pm$0.5 & 69.19$\pm$0.4 & \textbf{72.77}$^{**}\pm$0.2\\
                               & Large &  \cellcolor{apricot} 77.91 & 69.53$\pm$0.2 & \underline{70.43}$\pm$0.6 & 69.11$\pm$1.2  & 68.86$\pm$0.5 &  69.25$\pm$0.6 & 68.92$\pm$0.6 & \textbf{71.03}$^{*}\pm$0.3\\
        \bottomrule
    \end{tabular}
}
    \label{tab:main_res}
\end{table*}

==> table/main_res_gpt.tex <==
\begin{table*}[!htb]
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \textbf{Word Count} & \textbf{R1} &\textbf{R2} &\textbf{RL} &\textbf{RLSum} & \textbf{RM WR (\%)} \\
\midrule
 \multicolumn{7}{c}{
 \textbf{TL-DR} \quad  | T-S WR = 60.80
 } \\ 
\hline
Teacher& 25.81&	29.64&	8.82	&22.22	&22.22	&15.35 \\
Initial Student & 26.35&	29.04&	8.34&	21.66&	21.67&	11.51 \\
SFT Student &25.88&	29.08&	8.44&	21.76&	21.76&	11.40 \\
Standard KD & 26.50 &  & - & - & - & 12.47 \\
SeqKD&   26.14&  & & - & - & 13.18 \\
f-distill & 25.73 &  & - & - & - & 13.55\\
MiniLLM &  &  & - & - & - & - \\
Ours& 25.77 &  & - & - & - & 14.76 \\
\midrule
 \multicolumn{7}{c}{
 \textbf{Anthropic-HH}  | T-S WR = 55.23
 } \\ 
\hline
Teacher & 72.55	&21.47&	4.12&	13.66	&14.45&	15.52\\
Initial Student &73.53	&19.77&	3.36&	12.67&	13.46&	8.73  \\
SFT Student & 73.49&	18.51&	2.76&	11.93&	12.62&	8.79 \\
Standard KD & 73.09 & - & - & &  & 8.94  \\
SeqKD & 73.11 & - & - & - & - & 9.25 \\
f-distill & 72.68 &  & - & - & - & 9.66 \\
MiniLLM & - &  & - & - & - & - \\
Ours& 72.76 &  & - & - & - &  10.38\\
\bottomrule
\end{tabular}
\caption{Main results with the GPT-Neo model family. The teacher model is GPT-Neo-2.7B, and the student model is GPT-Neo-1.3B. WR stands for win rate, RM refers to a task-specific reward model, and AutoSxS refers to using a GPT-4 model for evaluation.}
\label{tab:res_gpt}
\end{table*}


==> table/main_res_llama.tex <==
\begin{table*}[!htb]
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \textbf{Word Count} & \textbf{R1} &\textbf{R2} &\textbf{RL} &\textbf{RLSum} & \textbf{RM WR (\%)}  \\
\midrule
 \multicolumn{7}{c}{
 \textbf{TL-DR} \quad  | T-S WR = 64.86
 } \\ 
\hline
Teacher & 25.51	& 33.14 & 11.4 & 25.31 & 25.31	& 45.28 \\
Initial Student & 27.24&	26.68&	8.98&	20.60&	20.15&	33.42\\
SFT & 25.77&	30.06&	9.95&	22.97&	22.97&	35.13 \\
Standard KD & 26.32 & - & - & - & - & 37.70 \\
SeqKD & 25.67 & - & - & - & - & 37.92 \\
f-distill & 25.98 &  & - & - &  & 38.35\\
MiniLLM & - &  & - & - & - & - \\
Ours& 26.02 & 31.46 & 10.79 & 24.65 & 24.65 & 40.46 \\
\midrule
 \multicolumn{7}{c}{
 \textbf{Anthropic-HH} \quad | T-S WR = 53.32
 } \\ 
\hline
Teacher & 67.78 &  25.15 & 6.50 & 16.32 & 17.12 & 26.95 \\
Initial Student & 67.80 &  24.96 & 6.48 & 16.26 & 17.05 & 25.63 \\
SFT Student & 67.64 &  25.33 & 6.66 & 16.51 & 17.28 & 25.52 \\
Standard KD & 67.60 & - & - & - & - & 25.83 \\
SeqKD & 67.73 & - & - & - & - & 26.24 \\
f-distill & 68.24 &  & - & - & - & 25.98 \\
MiniLLM & - &  & - & - & - & - \\
Ours& 67.93 & 25.54 & 6.82 & 16.70 & 17.33 & 27.74 \\
% \midrule
%  \multicolumn{7}{c}{
%  \textbf{Alpaca-GPT4} \quad Teacher WR = | Student WR = | T-S WR = 
%  } \\ 
% \hline
% SFT & 20 &  35.10 & 12.87 & 26.81 & 68.51 & - \\
% Standard KD & 20 & - & - & - & - & - \\
% SeqKD & 20 & - & - & - & - & - \\
% f-distill & 20 & - & - & - & - & - \\
% MiniLLM  & 20 & - & - & - & - & - \\
% Ours &  20 & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Main results with the LLaMA model family. The teacher model is LLaMA-2-13B, and the student model is LLaMA-2-7B. WR stands for win rate, RM refers to a task-specific reward model.}
\label{tab:res_llama}
\end{table*}


==> table/main_res_trans.tex <==
\begin{table*}[!th]
     % \vspace{-10pt}
    \centering
    \scalebox{.85}{
\begin{tabular}{l|cccccc|c}\toprule
       \multirow{2}{*}{Method}& \multirow{2}{*}{CoLA} & \multirow{2}{*}{MNLI} & \multirow{2}{*}{MRPC} & \multirow{2}{*}{RTE} & \multirow{2}{*}{SST-2} & \multirow{2}{*}{BoolQ}   & \multirow{2}{*}{Average} \\[0.75ex]
        & (Matt.) & (Acc.) & (F1) & (Acc.) & (Acc.) & (Acc.)  \\
        \midrule        
        Teacher T5-xxl  (\#Param. = 11B)& 71.5  &  94.7 & 92.4  & 92.2  & 96.4  & 89.1  & 89.4 \\
        \midrule
        Standard KL & 58.8  & 90.3  & 88.3  & 78.1  & 89.2  &  69.5 &  79.0  \\
        Temp. Scaling \citep{hinton2015distilling} &  59.4 & 90.7  & 88.9  & 79.6  &  89.4 & \underline{72.0}  &  80.0 \\
        Label Smoothing \citep{szegedy2016rethinking}&  59.3 & 90.6  & 89.2  & 79.2  & 89.9  & 68.6  & 79.6  \\
        Focal \citep{lin2017focal} & 59.2  & 90.7  &  88.7 &  80.4 & 89.3  & 68.2  & 79.6  \\
        Flooding \citep{ishida2020we} &  58.9 &  90.6 & 89.6  & 80.2  &  89.3 &  69.3 & 79.7  \\
        CRD \citep{tian2019contrastive}& 59.5  & 90.5  & 90.6  &  81.1 &  \underline{89.6} & 71.8  & 80.5 \\
        Annealing KD \citep{jafari2021annealing} &  59.8 & 90.7  & 90.0  &  80.7 & 89.3 & 70.7  &  80.2\\
        FilterKD \citep{ren2022better} & 59.2  & 90.7  & 89.5  &  80.4 & 89.3  & 69.6  & 79.8 \\
        MetaDistill \citep{zhou2022bert} & \underline{60.4}  & \underline{90.8}  & \textbf{91.4}  & \underline{81.3}  & 89.5  & 71.9  & \underline{80.9} \\
        \textbf{\ours (ours)} &  \textbf{61.2}  & \textbf{91.1}  & \underline{91.2}  &  \textbf{83.5} & \textbf{90.3}  &  \textbf{73.1} & \textbf{81.8 }\\
        \midrule
        \midrule
        Teacher T5-large (\#Param. = 770M) & 61.4  & 93.6  & 92.1  &  87.2 & 95.5  & 77.9  & 84.6\\
        \midrule
        Standard KL &  54.8 &  90.0 & 87.8  &  77.6 & 88.8  & 69.5  &  78.1 \\
        Temp. Scaling \citep{hinton2015distilling} &  55.6 & 90.4   & 88.7  & 79.4  & 89.2  & 70.4  &  79.1\\
        Label Smoothing \citep{szegedy2016rethinking}&  56.4 & 90.6  & 89.2  &  79.2 & 89.2  &  69.1 & 79.1 \\
        Focal \citep{lin2017focal} &  56.0  & 90.3  & 88.4 &  79.9 & 89.3  & 68.9  &  78.8\\
        Flooding \citep{ishida2020we} &   57.8  & 90.0  & 89.5 &  79.5  & 89.0  & 68.9  &  79.3\\
        CRD \citep{tian2019contrastive}&  58.2 & 90.2  & \underline{89.8}  &  80.3 &  \underline{89.4} & \underline{70.5}  & 79.7  \\
        Annealing KD \citep{jafari2021annealing} & 58.3  & 90.4  & \underline{89.8}  & 79.9  &  \underline{89.4} & 69.7  & 79.6 \\
        FilterKD \citep{ren2022better} &  56.7 & 90.2  &  89.1 & 78.8  &  89.2 & 69.2  & 78.9 \\
        MetaDistill \citep{zhou2022bert} & \underline{58.6}  & \textbf{90.7}  & 89.6  & \underline{81.0}  & 89.3  & 70.4  & \underline{80.1} \\
        \textbf{\ours (ours)} &  \textbf{60.5} & \textbf{90.7}  &  \textbf{91.1} & \textbf{82.7}  & \textbf{90.0}  & \textbf{71.0}  &  \textbf{81.0}\\
        \midrule
    \end{tabular}
}
     \caption{Main results on natural language datasets. The student model (BERT-base) is distilled from teacher models of different sizes (T5-xxl and T5-large). All results are averaged over three runs. The bolded numbers indicate the best results, while the underscore ``$\_$'' denotes the second-best results.
     }
    \label{tab:main_res}
\end{table*}

==> table/multi_class.tex <==
\begin{table}[!htb]
    \centering
     \caption{Results on a multi-class dataset ANLI.}
    \scalebox{1.0}{
    \begin{tabular}{c|c|c|c|c}\toprule
         ANLI& Run 1 & Run 2 & Run 3 & Average \\\midrule
         KL& 43.75&42.91 & 46.00& 44.22 \pm 1.60\\
         \ours& 46.25&  49.67 &  47.08 & 47.67 \pm1.78\\\bottomrule
    \end{tabular}
}
    \label{tab:anli}
\end{table}

==> table/reg_para.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|cc|cc|cc|cc|cc}\toprule
        Architecture & $\epsilon_1$ &$\epsilon_2$ &  $\epsilon_3$ & $\epsilon_4$ &  $\epsilon_5$ &$\gamma_1$ &  $\gamma_2$ & $\gamma_3$ &$\gamma_4$ &  $\gamma_5$\\\midrule
        xxl & 9.60& 5.44&  3.19& 0.93& 6.32&  8.64&  1.12& 2.35& 0.44& -0.75\\
        xl& 7.51& 1.81& 1.28& 0.08& 9.71& 9.87& 1.94& -0.62& -0.12& -0.62 \\
        large & 8.34& 1.41& 4.86& -0.61& -0.18&9.62& 8.86& 3.02& 5.94& 6.46\\\bottomrule
    \end{tabular}
    \caption{Searched perturbation coefficients using the equivalent-teacher method.}
    \label{tab:reg_para}
\end{table}

==> table/teacher_stats.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|ccccc}\toprule
         & Teacher Acc. & Validation TVD & Validation Log-loss & Student Acc. & Student PKD loss \\\midrule
       Teacher\_12  &84.03&	0.15&	1.69&	0.84&	0.51&	84.72&	0.49&	\\
       Teacher\_2  &  &&&&\\
       Teacher\_3  &  &&&&\\
       Teacher\_4  &  &&&&\\
       Teacher\_5  &  &&&&\\\bottomrule
    \end{tabular}
    \caption{Teacher statistics v.s. student performance.}
    \label{tab:teacher_stats}
\end{table}

==> table/ts_wr.tex <==
\begin{table}[!htb]
\centering
\begin{tabular}{ccc}
\toprule
 & \textbf{TL;DR} & \textbf{Anthropic-HH} \\\hline
LLaMA-2 & 64.86 & 53.97\\
GPT-Neo&  60.80 & 55.23\\
\bottomrule
\end{tabular}
\caption{Teacher-student win rate.}
\label{tab:ulm_res}
\end{table}

